A Penny for Your (visual) Thoughts: Self-Supervised Reconstruction of Natural Movies from Brain Activity

Reconstructing natural videos from fMRI brain recordings is very challenging, for two main reasons: (i) As fMRI data acquisition is difficult, we only have a limited amount of supervised samples, which is not enough to cover the huge space of natural videos; and (ii) The temporal resolution of fMRI recordings is much lower than the frame rate of natural videos. In this paper, we propose a self-supervised approach for natural-movie reconstruction. By employing cycle-consistency over Encoding-Decoding natural videos, we can: (i) exploit the full framerate of the training videos, and not be limited only to clips that correspond to fMRI recordings; (ii) exploit massive amounts of external natural videos which the subjects never saw inside the fMRI machine. These enable increasing the applicable training data by several orders of magnitude, introducing natural video priors to the decoding network, as well as temporal coherence. Our approach significantly outperforms competing methods, since those train only on the limited supervised data. We further introduce a new and simple temporal prior of natural videos, which - when folded into our fMRI decoder further - allows us to reconstruct videos at a higher frame-rate (HFR) of up to x8 of the original fMRI sample rate.

==> Guy_intro_May18_1930.tex <==

\section{Introduction}
% - Brain decoding is interesting and useful. 
Decoding observed natural visual stimuli from brain activity may be a cornerstone for brain-machine interfaces and for understanding visual processing in the brain. 
%
In particular, many works focused on the task of natural-image reconstruction from fMRI\footnote{functional magnetic resonance imaging.}-recorded brain activity \cite{Gaziv2022, Beliy2019, Cowen2014, Kamitani2005, Kay2009,Naselaris2009,Seeliger2018,Shen2019}. These works made strides in static stimulus reconstruction. However,  natural movies provide a closer, more realistic analog to dynamic visual experience~\cite{Nishimoto2011, Wen2018, Wang2022, Le2021}. The goal in this task is to develop a model that accurately reconstructs unknown natural movies from a subject's brain activity, which was recorded via fMRI while watching them (Fig~1). To this end, only a handful of data is provided: A dataset of 2.4hr video, comprising hundreds of few-sec video clips, and its associated fMRI recordings (``paired'' data).   
% making natural-movie reconstruction from fMRI a desirable goal~\cite{Nishimoto2011, Wen2018, Wang2022, Le2021} (Fig~1).

% challenges 
Reconstructing natural movies from fMRI is significantly more challenging than natural-image reconstruction. Specifically, adding the temporal dimension gives rise to two major additional challenges: (i)~The training data in current video-fMRI datasets is limited compared to the space of natural videos and possible fMRI recordings; (ii)~The temporal resolution of the fMRI recordings is low compared to the presented videos. While the latter is presented at a high frame-rate of 30 frames per second, the fMRI has a much lower temporal sampling rate of one sample every 2 seconds (i.e., 0.5Hz). Thus, each fMRI sample is influenced by tens of video frames. In contrast, image-fMRI datasets largely guarantee a one-to-one correspondence between an fMRI sample and its underlying single image. 
%
Moreover, fMRI data are based on slow oxygenated blood flow. This signal's relation to the underlying brain activity is formally given by the Haemodynamic Response Function (HRF), which has a temporal support of more than a dozen seconds, with a peak after about 4 seconds. This results in a severe loss of high temporal frequencies, and also video-fMRI misalignment issues. This poses additional challenges to recovering fast temporal information, and specifically to reconstructing movies with frame rate higher than the fMRI sample rate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Related works
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \vspace{-0.3cm}
% \textit{\textbf{Prior work on visual stimulus reconstruction from fMRI}} can be classified to still images vs. dynamic natural movies. Until recently, both types of visual reconstruction used a linear mapping between the fMRI data to image features (\cite{Kay2009, Naselaris2009, Shen2019, Guclu, Wen2018, Nishimoto2011}. In recent years, a few works found a strong correlation between features of convolutional neural networks (CNN) layers and brain activities of the visual cortex \cite{Kriegeskorte2015, Yamins2013}. That led to an increasing amount of work that used end-to-end CNN architectures to reconstruct the visual input \cite{Gaziv2022, Shen2019, Shen2019b, Gaziv2021, Wang2022, Han2019}. 

% video reconstruction with fMRI sample rate vs. fast reconstructions
\textit{\textbf{Prior work on natural-movie reconstruction from fMRI}} can be broadly classified to X families: (i)~Linear regression between fMRI data and hand-crafted video-features (e.g., motion-energy filters)~\cite{Nishimoto2011}. (ii) Linear regression between fMRI data and \underline{deep} (CNN-based) image or video features (e.g., using pretrained AlexNet)~\cite{Wen2018} 

focused on supervised methods using the ``paired'' data.


was inspired by natural-image reconstruction. It thus, mostly focused on a single frame-based reconstruction scheme that does not benefit from the 
The works on dynamic movies, however, neglected the temporal dimension and mostly reconstruct in a frame-based manner. A recent work of \cite{Wang2022} added a temporal constraint. To date, most of movie-based works have used supervised learning methods only. This means they were restricted to the sparse "paired" data. The first line of research has focused on reconstructing videos at a frame rate similar to that of fMRI \cite{Wen2018, Han2019, Le2021}. As an example, \cite{Wen2018} reconstructed the dynamic stimuli by learning a linear mapping between fMRI signal and deep feature maps. Later work by Han et. al. \cite{Han2019}, presented a variational auto-encoder, which learns a latent representation of the video frames, using Encoder \& Decoder networks. A linear mapping is then learned between the BOLD signal and the learned latent space. Finally the pre-trained decoder is used to reconstruct the frame out of the embedded BOLD signal. However, neither of the works considered the temporal dimensions of the data. Instead, it only used mapping from a single video frame to a single fMRI sample and back. An alternative line of research focuses on reconstructing video with a frame rate higher than that of fMRI. For example, \cite{Nishimoto2011} introduced learning based on a posterior probability of a video clip, given an fMRI sample. Thus, for an unseen fMRI sample, the reconstructed clip was another clip, taken from the training data, which had the highest probability given the unseen sample. Unlike most other works, this work uses real videos rather than reconstructing them from scratch. A more recent work \cite{Wang2022} used a conditional generative adversarial network (GAN). They used a temporal discriminator that determined the probability of a sequence to be the real sequence, given an fMRI sample. The temporal discriminator provided a temporal constraint, and with it, they succeeded in reconstructing videos 8 times faster than the fMRI sample rate. However, conditional GAN tends to overfit the training data and does not generalize well to "unseen" samples (i.e. not part of the training set). Hence, it can only train using pairs of fMRI recordings and their corresponding clips. Due to the limited training data, this method is not very generalizable. 


% \textit{\textbf{Prior work on natural-movie reconstruction from fMRI}} was inspired by natural-image reconstruction. It thus, mostly focused on a single frame-based reconstruction scheme that does not benefit from the 
% The works on dynamic movies, however, neglected the temporal dimension and mostly reconstruct in a frame-based manner. A recent work of \cite{Wang2022} added a temporal constraint. To date, most of movie-based works have used supervised learning methods only. This means they were restricted to the sparse "paired" data. The first line of research has focused on reconstructing videos at a frame rate similar to that of fMRI \cite{Wen2018, Han2019, Le2021}. As an example, \cite{Wen2018} reconstructed the dynamic stimuli by learning a linear mapping between fMRI signal and deep feature maps. Later work by Han et. al. \cite{Han2019}, presented a variational auto-encoder, which learns a latent representation of the video frames, using Encoder \& Decoder networks. A linear mapping is then learned between the BOLD signal and the learned latent space. Finally the pre-trained decoder is used to reconstruct the frame out of the embedded BOLD signal. However, neither of the works considered the temporal dimensions of the data. Instead, it only used mapping from a single video frame to a single fMRI sample and back. An alternative line of research focuses on reconstructing video with a frame rate higher than that of fMRI. For example, \cite{Nishimoto2011} introduced learning based on a posterior probability of a video clip, given an fMRI sample. Thus, for an unseen fMRI sample, the reconstructed clip was another clip, taken from the training data, which had the highest probability given the unseen sample. Unlike most other works, this work uses real videos rather than reconstructing them from scratch. A more recent work \cite{Wang2022} used a conditional generative adversarial network (GAN). They used a temporal discriminator that determined the probability of a sequence to be the real sequence, given an fMRI sample. The temporal discriminator provided a temporal constraint, and with it, they succeeded in reconstructing videos 8 times faster than the fMRI sample rate. However, conditional GAN tends to overfit the training data and does not generalize well to "unseen" samples (i.e. not part of the training set). Hence, it can only train using pairs of fMRI recordings and their corresponding clips. Due to the limited training data, this method is not very generalizable. 

 

% Our work
We present a new approach for natural-movie reconstruction that handles the lack of training data. 
%
Our approach directly leverages upon the abundance of training data provided by the \underline{many} frames of the \underline{high frame-rate video}, relative to the \underline{much fewer} frames given by the low frame-rate recorded fMRI~(Fig~1). We achieve this by introducing \textit{self-supervised training on \underline{unpaired} videos (videos with no fMRI recordings).} 
%
Our approach is illustrated in Fig~\ref{train fig}. We train two types of deep neural networks: an Encoder E, which predicts a single fMRI frame given a 2-sec input video clip~(Fig~\ref{train fig}a), and a Decoder D, which reconstructs a single video frame from an fMRI frame~(Fig~\ref{train fig}b). Composing those two networks, E-D, yields a combined network whose input and output are video frames, and enables to impose a cycle-consistency criterion between the middle-input and the output frames for \underline{arbitrary} video data~(Fig~\ref{train fig}c). 
%
% Notably, this training configuration does not require any fMRI recording, and may apply to any natural movie data. 
Specifically, we use this self-supervised criterion to \textit{train on (i)~Video clips from the training data that do not have corresponding fMRI ("Internal data"), and (ii)~Natural video clips that are external to the fMRI dataset ("External data")}. Applying this to \underline{partially overlapping video clips}, expands the training data by several orders of magnitude, owing to the high frame-rate of the video~(Fig~\ref{train fig}d). The benefit of this approach is two-fold: (i)~It better exploits the internal, readily available training data, and (ii)~Training on partially overlapping clips improves learning of temporal dynamics. Altogether, this results in a leap improvement in reconstruction quality over the supervised-only approach~(Fig~\ref{train fig}e), and in state-of-the-art reconstruction results~(Fig~3).
%
In addition, we developed a novel natural temporal prior that enables to reconstruct videos at up to x8 of the original fMRI frame-rate with accurate temporal dynamics details.  

Adding self-supervision on unpaired data was previously proposed in the context of natural image reconstruction~\cite{Gaziv2022,Beliy2019}. However, their approaches heavily relied on large \underline{external} natural-image datasets for self-supervised training. Our self-supervision for video reconstruction is significantly different. Firstly, unlike image-fMRI datasets, where there is full (1:1) image-fMRI correspondence, in video-fMRI datasets there are many frames in the training data with no corresponding fMRI. These provide massive training data expansion by applying self-supervision \underline{internally} -- giving rise to a leap improvement in reconstruction quality -- even without resorting to external datasets. Secondly, the consecutive frames in natural \underline{videos} are strongly correlated, representing an additional layer of valuable temporal dynamics information, which does not exist in the natural \underline{images} case. 

Reconstructing natural videos at a faster frame-rate than the fMRI's was previously proposed in~\cite{Wang2022}. However here, we propose a novel temporal prior that, when incorporated into training, gives rise to additional temporal dynamics details over~\cite{Wang2022}.

% %
% Further, we introduce a novel temporal constraint, within the same reconstruction, and over consecutive reconstructions. A self-supervised temporal representation of the training data is learned, and successive reconstruction is enforced to be close to their ground truth representations. These two criteria are used to reconstruct temporally contiguous and detailed video clips with a higher frame rate than of the captured fMRIs (see figure \ref{decoder 1Hz fig}).

\underline{Our contributions are therefore several-fold: }
\newline \ 
$\bullet$
We propose a new self-supervised approach to handle the inherent lack of training data in natural movie reconstruction from fMRI.
\newline \ 
$\bullet$
State-of-the-art natural-movie reconstruction quality from fMRI.
\newline \ 
$\bullet$
We propose a new temporal dynamics prior that allows to reconstruct videos at a higher frame-rate than the fMRI's with accurate temporal dynamics details.
 
% \underline{Our contributions are therefore several-fold: }
% \newline \ 
% $\bullet$
% A self-supervised approach to handle the inherent lack in  ``paired'' fMRI-movie training data.
% \newline \ 
% $\bullet$
% State-of-the-art results in natural-movie reconstruction from fMRI.
% % \newline \ 
% % $\bullet$
% % A self-supervised temporal prior on natural videos. 
% %that allows to reconstruct videos at a higher frame-rate than the fMRI's with accurate temporal dynamics details.
% \newline \ 
% $\bullet$
% {High Frame-Rate (HFR) video reconstruction -- higher than the underlying fMRI sampling rate.}

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
      \answerNA{Decoding fMRI information is a problem which has been researched for more than a decade. We extended the envelope with additional layer of temporal information}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All instructions to reproduce our results are included as well as references to the publicly available datasets that we used. We will make our algorithm code publicly available upon publication.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{We included full citation and references to the sources of the code and the datasets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{We will make our algorithm code publicly available upon publication.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We used publicly available fMRI datasets, released by others.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We used publicly available fMRI datasets, collected and published previously.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}




==> introduction_bak.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INTRODUCTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ganit (27.4.22)

\section{Introduction}
% - Brain decoding is interesting and useful. 
 Decoding natural visual stimuli from recorded brain activity has gained a lot of attention in recent years. This is because understanding visual processes can be useful for many applications. For example, enabling more accurate diagnosis and communication with patients in a vegetative or minimally conscious state \cite{Naci2012, Milekovic2018, Kubler2013}, detecting covert attention \cite{Ahmadi2020, Ekanayake2018}, and even understanding mental imagery \cite{Cichy2012, Naselaris2015, Pearson2015, Horikawa2013, Horikawa2017}. A particularly interesting task that drew attention is the decoding of visual stimuli from fMRI recordings. To date, most work has focused mainly on the reconstruction of natural images \cite{Gaziv2022, Beliy2019, Cowen2014, Kamitani2005, Kay2009,Naselaris2009,Seeliger2018,Shen2019}. While these works made strides in static stimulus reconstruction, natural movies provide a closer, more realistic analog to dynamic visual experience~\cite{Nishimoto2011, Wen2018, Wang2022, Le2021}. 

% challenges 
Natural-movie reconstruction from fMRI is significantly more challenging than natural-image reconstruction, due to the addition of temporal dimension. In particular, two major challenges arise from natural-movies. The first challenge is the limited data in current datasets compared to the dimensionality of the data. The second challenge arises from the low temporal resolution of the fMRI signals. While the presented videos have a frame rate of around 30 frames per second, the fMRI has a much lower temporal sampling rate of one sample every 2 seconds (i.e. 0.5Hz). Thus, each fMRI sample is influenced by tens of video frames. This stands, in contrast, to still image experiments, in which each fMRI sample is influenced mainly from a single image. Moreover, the fMRI is measuring the hemodynamic response function (HRF). This functions' temporal support spreads over more than 10 seconds, with a peak after around 5 seconds. This means that the HRF acts as a severe temporal low pass filter, further reducing the temporal resolution. Thus, when measuring the hemodynamic response, there is a major loss of temporal information. These challenges make it difficult to reconstruct movies with frame rate higher than the fMRI sample rate.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Related works
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-0.3cm}
\subparagraph{Prior works}
% reconstruction of visual stimuli
on visual stimulus reconstruction from fMRI can be classified to still images vs. dynamic natural movies. Until recently, both types of visual reconstruction used a linear mapping between the fMRI data to image features (\cite{Kay2009, Naselaris2009, Shen2019, Guclu, Wen2018, Nishimoto2011}. In recent years, a few works found a strong correlation between features of convolutional neural networks (CNN) layers and brain activities of the visual cortex \cite{Kriegeskorte2015, Yamins2013}. That led to an increasing amount of work that used end-to-end CNN architectures to reconstruct the visual input \cite{Gaziv2022, Shen2019, Shen2019b, Gaziv2021, Wang2022, Han2019}. 

% video reconstruction with fMRI sample rate vs. fast reconstructions
The works on dynamic movies, however, neglected the temporal dimension and mostly reconstruct in a frame-based manner. A recent work of \cite{Wang2022} added a temporal constraint. To date, most of movie-based works have used supervised learning methods only. This means they were restricted to the sparse "paired" data. The first line of research has focused on reconstructing videos at a frame rate similar to that of fMRI \cite{Wen2018, Han2019, Le2021}. As an example, \cite{Wen2018} reconstructed the dynamic stimuli by learning a linear mapping between fMRI signal and deep feature maps. Later work by Han et. al. \cite{Han2019}, presented a variational auto-encoder, which learns a latent representation of the video frames, using Encoder \& Decoder networks. A linear mapping is then learned between the BOLD signal and the learned latent space. Finally the pre-trained decoder is used to reconstruct the frame out of the embedded BOLD signal. However, neither of the works considered the temporal dimensions of the data. Instead, it only used mapping from a single video frame to a single fMRI sample and back. An alternative line of research focuses on reconstructing video with a frame rate higher than that of fMRI. For example, \cite{Nishimoto2011} introduced learning based on a posterior probability of a video clip, given an fMRI sample. Thus, for an unseen fMRI sample, the reconstructed clip was another clip, taken from the training data, which had the highest probability given the unseen sample. Unlike most other works, this work uses real videos rather than reconstructing them from scratch. A more recent work \cite{Wang2022} used a conditional generative adversarial network (GAN). They used a temporal discriminator that determined the probability of a sequence to be the real sequence, given an fMRI sample. The temporal discriminator provided a temporal constraint, and with it, they succeeded in reconstructing videos 8 times faster than the fMRI sample rate. However, conditional GAN tends to overfit the training data and does not generalize well to "unseen" samples (i.e. not part of the training set). Hence, it can only train using pairs of fMRI recordings and their corresponding clips. Due to the limited training data, this method is not very generalizable. 


% Our work
We present a novel method for self-supervised reconstruction of natural movies, which leverage much more data. Our method allows to reconstruct at the captured fMRI-rate (0.5Hz) or even higher (up to 4Hz, which is x8 faster). For this purpose, we train two separate models: an encoder (E) that maps a short video clip into an fMRI sample (see figure \ref{train fig}a), and a decoder (D) that maps fMRI samples into reconstructed video frames (see figure \ref{train fig}b,d). By concatenating these two networks, encoder-decoder, we get a single network E-D whose input and output are video frames, hence, does not require any fMRI recording (see figure \ref{train fig}c,e). Therefore, we can vastly widen the supervised training set, since we can train on \underline{unpaired} videos without fMRI. Reconstruction examples can be seen in figure \ref{decoder nice reconst}. Further, we introduce a novel temporal constraint, within the same reconstruction, and over consecutive reconstructions. A self-supervised temporal representation of the training data is learned, and successive reconstruction is enforced to be close to their ground truth representations. These two criteria are used to reconstruct temporally contiguous and detailed video clips with a higher frame rate than of the captured fMRIs (see figure \ref{decoder 1Hz fig}).

Our contributions are therefore several-fold: (1) We propose a new approach to handle the inherent lack in Movie-fMRI training data. (2) State-of-the-art natural movie-reconstruction quality from fMRI. (3) We demonstrate reconstruction capabilities at a frame-rate higher than the fMRIs' sample-rate with consistent temporal dynamics.
 

% % Ganit (24.4.22)

% \section{Introduction}
% % - Brain decoding is interesting and useful. 
%  Decoding natural visual stimuli from recorded brain activity has gained a lot of attention in recent years. This is because understanding neural processes can be useful for many aspects. For example, enabling more accurate diagnosis and communication with patients in a vegetative or minimally conscious state \cite{Naci2012, Milekovic2018, Kubler2013}, detecting covert attention \cite{Ahmadi2020, Ekanayake2018}, and even understanding mental imagery \cite{Cichy2012, Naselaris2015, Pearson2015, Horikawa2013, Horikawa2017}. A particularly interesting task that drew attention is that of decoding visual stimuli from fMRI recordings. To date, most work has focused mainly on the reconstruction of natural images \cite{Gaziv2022, Beliy2019, Cowen2014, Kamitani2005, Kay2009,Naselaris2009,Seeliger2018,Shen2019}. While these works made strides in static stimulus reconstruction, natural movies provide a closer, more intuitive analog to dynamic visual experience~\cite{Nishimoto2011, Wen2018, Wang2022, Le2021}. 

% % challenges 
% Natural-movie reconstruction from fMRI is particularly challenging, even beyond natural-image reconstruction, due to adding the temporal dimension. The first one is to acquire sufficient data of natural movies and the corresponding fMRI recordings to span the huge space of natural videos. The second challenge arises from the low temporal resolution of the fMRI signals. While the presented videos have a frame rate of around 15 frames per second, the fMRI has a temporal resolution of one sample every 2 seconds. Thus, each fMRI sample is influenced by tens of video frames. This stands, in contrast, to still image experiments, in which each fMRI sample is influenced by a single image. Moreover, the fMRI is measuring the hemodynamic response function (HRF). This functions' temporal response spreads over 10 seconds, with a peak after around 5 seconds. This means that the HRF acts as a temporal low pass filter. Thus, when measuring the hemodynamic response, there is a major loss of temporal information. These challenges make it difficult to reconstruct movies with frame rate higher than the fMRI sample rate.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Related works
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{figure}[H]%
%         \centering
%         \subfloat{{\includegraphics[width=\textwidth]{figs/0.5Hz reconst fig - best sub.pdf} }}%
        
%         \caption{\textbf{Decoder - 0.5 Hz reconstruction examples - } comparison between the original and reconstructed frames. The first row shows the "ground truth" video frames. The second row shows reconstructions from subject 2}
%         \label{decoder nice reconst}%
        
%     \end{figure}


% \subparagraph{Prior works}
% % reconstruction of visual stimuli
% on visual stimulus reconstruction from fMRI can be classified to still images vs. dynamic natural movies. Up until recently, both types of visual reconstruction used learning the linear mapping between the fMRI data to image features (\cite{Kay2009, Naselaris2009, Shen2019, Guclu, Wen2018, Nishimoto2011}. In recent years, a few works found a strong correlation between features of convolutional neural networks (CNN) layers and brain activities of the visual cortex \cite{Kriegeskorte2015, Yamins2013}. That led to an increasing amount of work that used end-to-end CNN architectures to reconstruct the visual input \cite{Gaziv2022, Shen2019, Shen2019b, Gaziv2021, Wang2022, Han2019}. The works on dynamic movies, however, neglected the temporal dimension and mostly reconstruct in a frame-based manner. A recent work of \cite{Wang2022} added a temporal constraint. To date, movie-based works have used supervised learning methods only. This means they were restricted to the sparse "paired" data.

% % video reconstruction with fMRI sample rate
% A first line of work has focused on reconstructing videos at a frame rate similar to that of fMRI \cite{Wen2018, Han2019, Le2021}. For instance, \cite{Wen2018} reconstructed the dynamic stimuli by learning a linear mapping between the observed fMRI signal and feature maps of the stimuli extracted using the first layer of AlexNet \cite{Krizhevsky2012}. With this method, however, they achieved only grayscale reconstruction of the RGB video frames. Later work by Han et. al. \cite{Han2019}, presented a variational auto-encoder, which learns a latent representation of the video frames, using Encoder \& Decoder networks. By using this architecture, they succeeded to reconstruct the RGB video frames out of the BOLD signal. This was done by learning a linear mapping between the BOLD signal and the learned latent space, which goes into the decoder model to obtain the reconstructed frame. The work of \cite{Han2019} used an expended dataset version of the previous work \cite{Wen2018}, with a much larger training set of 13.1h video clips (instead of 1.6h as in \cite{Wen2018}). Nonetheless, this work ignored the temporal dimension of the data, and in the learning process only used mapping from a single video frame to a single fMRI sample and back.  

% %  video reconstruction with temporal super resolution (add the point of conditional GAN is restricted to the training data)
% Another line of work has focused on the reconstruction of video with a frame rate higher than the one of the fMRI. For example, \cite{Nishimoto2011} introduced learning based on a posterior probability of a video clip, given an fMRI sample. Thus, for an fMRI sample taken with a clip not present in the training database, the reconstructed clip was taken from the training data, which had the highest probability given the unseen sample. This work, however, does not reconstruct the stimuli from scratch, but rather uses real natural videos. A more recent work \cite{Wang2022} used a conditional generative adversarial network (GAN). They used a temporal discriminator that determined the probability of a sequence to be the real sequence, given an fMRI sample. The temporal discriminator provided a temporal constraint, and with it they succeeded in reconstructing videos 8 times faster than the fMRI sample rate. However, conditional GAN tends to overfit the training data and does not generalize well to "unseen" samples (i.e. not part of the training set). Meaning that it can only train using pairs of fMRI recordings and their matching clips. Since one of the main challenges is the very limited training data, the generalization abilities of this method are very restrictive. 
%   \begin{figure}[H]%
%         \centering
%         \subfloat{{\includegraphics[width=\textwidth]{figs/2Hz - best sub.pdf} }}%

       
%         \caption{\textbf{Decoder - 2 Hz reconstruction examples - } comparison between the original and reconstructed frames from subject 2 fMRI recordings. 
%         \label{decoder 1Hz fig}}
        
        
%     \end{figure}
% % pre-trained action recognition network + self-supervised video representation
% For the task of video reconstruction, we wanted to benefit from pre-trained temporal features in addition to the spatial features. For this purpose, we examined works that focus on video comprehensions, such as video classification or action recognition. In those works, one needs to process the temporal information, in addition to processing the spatial information. Several works have tried to tackle these tasks using two-stream networks - one stream for RGB, and another one for optical flow (OF) \cite{Carreira2017, Stroud2020}. However, these methods require computing the OF in advance, which means that they are not end-to-end networks. Some recent works have tried to tackle these tasks using implicit learning of the motion. A recent work by \cite{Crasto2019}, trained two networks - a teacher network that learns action recognition using OF as an input, and a student network, that receives only RGB input (MARS network). The student network learns to classify actions based on the RGB input, and the teacher network outputs. At inference time the network uses only the RGB input, meaning that the network learns implicitly the motion input. In another line of work, a better implicit video representation was learned in a self-supervised manner (without manual labels), using a different task that focuses on the temporal dimension. For example, pace prediction \cite{Wang2020,  Benaim2020, Yao2020}, distinguishes between ordered and shuffled videos \cite{Misra2016, Fernando2017, Jenni2020} and prediction of the next frame \cite{DPC}. Those works succeed in achieving state-of-the-art results on action recognition and video classification tasks, by employing the implicit video representation they have learned.

% % Our work
% In the following work, we use a novel methods for self-supervision on natural movies, for reconstructing high-resolution videos, with faster frame rate than the fMRIs' sample rate. For this purpose, we train two different models - an encoder that maps a short video clip to an fMRI sample (see figure \ref{train fig}a), and a decoder that maps fMRI samples to reconstructed video frames (see figure \ref{train fig}b,d). When concatenating these two network together, encoder-decoder, we receive a single network that has similar input ad output (see figure \ref{train fig}c,e). With this network, we can extensively magnify the training set size, by training on unpaired videos. Moreover, by exploiting the temporal dimension of the data, we enforce temporal continuity over consecutive samples. This by enforcing consistency over temporal overlapping reconstructed frames (see figure \ref{train fig}f). Our contributions are therefore several-fold: (1) We propose a new approach to handle the inherent lack in Movie-fMRI training data. (2) State-of-the-art natural movie-reconstruction quality from fMRI. (3) We demonstrate reconstruction capabilities at a frame-rate higher than the fMRIs' sample-rate with consistent temporal dynamics.
 


% % Ganit (15.4.22)

% \section{Introduction}
% % - Brain decoding is interesting and useful. 
%  Learning to decode brain activity has gained interest in recent years. This is because understanding neural processes can be useful for many aspects. For example, enabling more accurate diagnosis and communication with patients in a vegetative or minimally conscious state \cite{Naci2012, Milekovic2018, Kubler2013}, detecting covert attention \cite{Ahmadi2020, Ekanayake2018}, and even understanding mental imagery \cite{Cichy2012, Naselaris2015, Pearson2015, Horikawa2013, Horikawa2017}. A particularly interesting task that drew attention is that of decoding visual stimuli from fMRI recordings. To date, most work has focused mainly on the reconstruction of natural images \cite{Gaziv2022, Beliy2019, Cowen2014, Kamitani2005, Kay2009,Naselaris2009,Seeliger2018,Shen2019}. While these works made strides in static stimulus reconstruction, natural movies provide a closer, more intuitive analog to dynamic visual experience~\cite{Nishimoto2011, Wen2018, Wang2022, Le2021}. 

% % challenges 
% Natural-movie reconstruction from fMRI is particularly challenging, even beyond natural-image reconstruction, due to adding the temporal dimension. The first one is to acquire sufficient data of natural movies and the corresponding fMRI recordings to span the huge space of natural videos. The second challenge arises from the low temporal resolution of the fMRI signals. While the presented videos have a frame rate of around 15 frames per second, the fMRI has a temporal resolution of one sample every 2 seconds. Thus, each fMRI sample is influenced by tens of video frames. This stands, in contrast, to still image experiments, in which each fMRI sample is influenced by a single image. Moreover, the fMRI is measuring the hemodynamic response function (HRF). This functions' temporal response spreads over 10 seconds, with a peak after around 5 seconds. This means that the HRF acts as a temporal low pass filter. Thus, when measuring the hemodynamic response, there is a major loss of temporal information. These challenges make it difficult to reconstruct movies with frame rate higher than the fMRI sample rate.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Related works
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subparagraph{Prior works}
% % reconstruction of visual stimuli
% on visual stimulus reconstruction from fMRI can be classified to still images vs. dynamic natural movies. Up until recently, both types of visual reconstruction used learning the linear mapping between the fMRI data to image features (\cite{Kay2009, Naselaris2009, Shen2019, Guclu, Wen2018, Nishimoto2011}. In recent years, a few works found a strong correlation between features of convolutional neural networks (CNN) layers and brain activities of the visual cortex \cite{Kriegeskorte2015, Yamins2013}. That led to an increasing amount of work that used end-to-end CNN architectures to reconstruct the visual input \cite{Gaziv2022, Shen2019, Shen2019b, Gaziv2021, Wang2022, Han2019}. The works on dynamic movies, however, neglected the temporal dimension and mostly reconstruct in a frame-based manner. A recent work of \cite{Wang2022} added a temporal constraint. To date, movie-based works have used supervised learning methods only. This means they were restricted to the sparse "paired" data.

% % video reconstruction with fMRI sample rate
% A majority of the research has focused on reconstructing videos at a frame rate similar to that of fMRI \cite{Wen2018, Han2019, Le2021}. For instance, \cite{Wen2018} reconstructed the dynamic stimuli by learning a linear mapping between the observed fMRI signal and feature maps of the stimuli extracted using the first layer of AlexNet \cite{Krizhevsky2012}. With this method, however, they achieved only grayscale reconstruction of the RGB video frames. Later work by Han et. al. \cite{Han2019}, presented a variational auto-encoder, which learns a latent representation of the video frames, using Encoder \& Decoder networks. By using this architecture, they succeeded to reconstruct the RGB video frames out of the BOLD signal. This was done by learning a linear mapping between the BOLD signal and the learned latent space, which goes into the decoder model to obtain the reconstructed frame. The work of \cite{Han2019} used an expended dataset version of the previous work \cite{Wen2018}, with a much larger training set of 13.1h video clips (instead of 1.6h as in \cite{Wen2018}). Nonetheless, this work ignored the temporal dimension of the data, and in the learning process only used mapping from a single video frame to a single fMRI sample and back.  

% %  video reconstruction with temporal super resolution (add the point of conditional GAN is restricted to the training data)
% Another line of work has focused on the reconstruction of video with a frame rate higher than the one of the fMRI. For example, \cite{Nishimoto2011} introduced learning based on a posterior probability of a video clip, given an fMRI sample. Thus, for an fMRI sample taken with a clip not present in the training database, the reconstructed clip was taken from the training data, which had the highest probability given the unseen sample. This work, however, does not reconstruct the stimuli from scratch, but rather uses real natural videos. A more recent work \cite{Wang2022} used a conditional generative adversarial network (GAN). They used two discriminators - spatial and temporal. The temporal discriminator received an fMRI sample and spatially downsampled 8-frames reconstructed sequence, and determined the probability that this sequence is the real sequence, given the fMRI sample. With the temporal discriminator, they succeeded in reconstructing videos 8 times faster than the fMRI sample rate. This work, however, did not enforced temporal contingency between successive reconstructions, which led to temporal discontinuity within the same reconstructed clip. Moreover, conditional GAN tends to overfit the training data and does not generalize well to "unseen" samples (i.e. not part of the training set). Meaning that it can only train using pairs of fMRI recordings and their matching clips. Since one of the main challenges is the very limited training data, the generalization abilities of this method are very restrictive. 
%   \begin{figure}[H]%
%         \centering
%         \subfloat{{\includegraphics[width=\textwidth]{Slide11.JPG} }}%
        
%         \caption{\textbf{Decoder - 0.5 Hz reconstruction examples - } comparison between the original and reconstructed frames. The first row shows the "ground truth" video frames. The 2-4th rows shows reconstructions from subjects 1-3 respectively}
%         \label{decoder nice reconst}%
        
%     \end{figure}

% % pre-trained action recognition network + self-supervised video representation
% For the task of video reconstruction, we wanted to benefit from pre-trained temporal features in addition to the spatial features. For this purpose, we examined works that focus on video comprehensions, such as video classification or action recognition. In those works, one needs to process the temporal information, in addition to processing the spatial information. Several works have tried to tackle these tasks using two-stream networks - one stream for RGB, and another one for optical flow (OF) \cite{Carreira2017, Stroud2020}. However, these methods require computing the OF in advance, which means that they are not end-to-end networks. Some recent works have tried to tackle these tasks using implicit learning of the motion. A recent work by \cite{Crasto2019}, trained two networks - a teacher network that learns action recognition using OF as an input, and a student network, that receives only RGB input (MARS network). The student network learns to classify actions based on the RGB input, and the teacher network outputs. At inference time the network uses only the RGB input, meaning that the network learns implicitly the motion input. In another line of work, a better implicit video representation was learned in a self-supervised manner (without manual labels), using a different task that focuses on the temporal dimension. For example, pace prediction \cite{Wang2020,  Benaim2020, Yao2020}, distinguishes between ordered and shuffled videos \cite{Misra2016, Fernando2017, Jenni2020} and prediction of the next frame \cite{DPC}. Those works succeed in achieving state-of-the-art results on action recognition and video classification tasks, by employing the implicit video representation they have learned.

% % Our work
% In the following work, we reconstruct the dynamic stimuli, by using novel methods for self-supervision. For this purpose, we use two different networks - an encoder that receives a short video clip and outputs an fMRI sample, and a decoder network that receives one or more fMRI samples and outputs one or more reconstructed video frames. By concatenating these two networks together, encoder-decoder, we obtain a single network, that receives a short video clip and outputs one or more frames. With the concatenated network, we can train the decoder network using clips that do not have matching fMRI. In particular, we can use clips out of the training clips, that are not aligned to any fMRI sample. Moreover, by exploiting the temporal dimension of the data, we enforce temporal continuity over consecutive samples. This by enforcing reconstruction consistency over overlapping (in time) reconstructed frames. 
% The main contributions of this work are: (1) training video decoder using self-supervision which is shown to improve the results of supervised approaches and other competing methods. (2) Reconstructions temporally consistent video with a higher frame rate relative to the fMRI sampling rate. 
%   \begin{figure}[H]%
%         \centering
%         \subfloat{{\includegraphics[width=\textwidth]{Slide15.JPG} }}%

%         \\
%         \subfloat{{\includegraphics[width=\textwidth]{Slide16.JPG} }}%
    
%         \caption{\textbf{Decoder - 1 Hz reconstruction examples - } comparison between the original and reconstructed frames. The 2-4th rows shows reconstructions from subjects 1-3 correspondingly
%         \label{decoder 1Hz fig}}
        
        
%     \end{figure}




% Ganit(12.4.22)
% \section{Introduction}
% % - Brain decoding is interesting and useful. 
% Learning to decode brain activity has gained interest in recent years. This is because understanding neural processes can be useful for many aspects. For example, enabling more accurate diagnosis and communication with patients in a vegetative or minimally conscious state \cite{Naci2012, Milekovic2018, Kubler2013}, detecting covert attention \cite{Ahmadi2020, Ekanayake2018}, and even understanding mental imagery \cite{Cichy2012, Naselaris2015, Pearson2015, Horikawa2013, Horikawa2017}. A particular interesting task that drew attention is the task of decoding visual stimuli from fMRI recordings. To this day, the research has focused mainly on the reconstruction of natural images \cite{Gaziv2022, Beliy2019, Cowen2014, Kamitani2005, Kay2009,Naselaris2009,Seeliger2018,Shen2019}. However, natural movies provide a closer, more intuitive analog to dynamic visual experience~\cite{Nishimoto2011, Wen2018, Wang2022, Le2021}. Therefore, reconstructing high-quality natural movies can significantly improve the current brain decoding applications.

% % challenges
% However, reconstructing videos from fMRI recordings presents several challenges. The first one is to acquire sufficient data of videos and the corresponding fMRI activities, that will span the huge space of natural videos. The second challenge arises from the low temporal resolution of the fMRI signals. While the presented videos have a frame rate of around 15 frames per second, the fMRI has a temporal resolution of one sample every 2 seconds. Thus, each fMRI signal is influenced by tens of video frames. This stands, in contrast, to still image experiments, in which each fMRI signal is influenced by a single image. Moreover, the fMRI is measuring the hemodynamic response function (HRF). This functions' temporal support spreads over 10 seconds, with a peak after around 5 seconds. This means that the HRF acts as a temporal low pass filter. Thus, when measuring the hemodynamic response, there is a dramatic loss of temporal information. These challenges make it difficult to reconstruct movies with consistent dynamics details that have a frame rate higher than the fMRI sample rate.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Related works
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subparagraph{Prior works}
% % reconstruction of visual stimuli
% Up until the recent years, visual reconstruction was done by learning the linear mapping between the fMRI data to either handcrafted image features (e.g., using Gabor wavelets) \cite{Kay2009,Naselaris2009} or deep image features (e.g., using pre-trained AlexNet) \cite{Shen2019, Guclu, Wen2018, Nishimoto2011}. However, in recent years, few works \cite{Kriegeskorte2015, Yamins2013} found a strong correlation between features of convolutional neural networks (CNN) layers and brain activities of the visual cortex. That led to an increasing amount of work that implemented end-to-end CNN architectures to reconstruct the visual input \cite{Gaziv2022, Shen2019, Shen2019b, Gaziv2021, Wang2022}. For example, a work that focused on natural images trained two separated networks - encoder network and decoder network \cite{Gaziv2022}. The encoder learned mapping from image to fMRI signal, and the decoder learned mapping from fMRI signal to image. This was done in a supervised manner, using labeled pairs of \{image, fMRI\}. Moreover, concatenating those two networks back-to-back, yielded a combined network that has the same input and output. This allowed training the network in a self-supervised manner on unpaired images.

%   \begin{figure}[H]%
%         \centering
%         \subfloat{{\includegraphics[width=\textwidth]{Slide11.JPG} }}%
        
%         \caption{\textbf{Decoder - 0.5 Hz reconstruction examples - } comparison between the original and reconstructed frames. The first row shows the ground truth video frames. The 2-4th rows shows reconstructions from subjects 1-3 respectively}
%         \label{decoder nice reconst}%
        
%     \end{figure}

% % video reconstruction with fMRI sample rate
% Several works have attempted the task of reconstructing dynamic stimuli from brain activity. A majority of the research has focused on reconstructing spatially competent videos at a frame rate similar to that of fMRI \cite{Wen2018, Han2019, Le2021}. For instance, Wen et. al. \cite{Wen2018}, reconstructed the dynamic stimuli by learning a linear mapping between the observed fMRI signal and feature maps of the stimuli extracted using the first layer of AlexNet \cite{Krizhevsky2012}. With this method, however, they achieved only grayscale reconstruction of the RGB video frames. Later work by Han et. al. \cite{Han2019}, learned a variational auto-encoder, that learns a latent representation of the video frames, using Encoder \& Decoder networks. By using these architectures, they succeeded to reconstruct the RGB video frames out of the BOLD signal. This was done by learning a linear mapping between the BOLD signal and the learned latent space, which goes into the Decoder model to obtain the reconstructed frame. This work used an expended dataset version of the previous work \cite{Wen2018}, with 13.1h of training clips, instead of 1.6h. Nonetheless, this work ignored the temporal dimension of the data, and only learned mapping from a single frame to fMRI and back.  

% %  video reconstruction with temporal super resolution (add the point of conditional GAN is restricted to the training data)
% Another line of work has focused on the reconstruction of temporally super-resolved video (i.e. with a frame rate higher than the one of the fMRI). For example, Nishimoto et al. \cite{Nishimoto2011} learned a posterior probability of a video clip, given an fMRI sample. Thus, for an unseen fMRI sample, the reconstructed clip was taken from the training data, which had the highest probability given the unseen sample. This work, however, does not reconstruct the stimuli from scratch, but rather uses real natural videos. A more recent work \cite{Wang2022} used a conditional generative adversarial network (GAN). They used two discriminators - spatial and temporal. The temporal discriminator received an fMRI sample and spatially downsampled 8-frames reconstructed sequence, and determined the probability that this sequence is the real sequence, given the fMRI sample. With the temporal discriminator, they succeeded in reconstructing videos 8 times faster than the fMRI sample rate. However, this work did not enforce consistency between consecutive fMRI samples, which led to temporal inconsistencies within the same reconstructed clip. Moreover, conditional GAN tends to overfit the training data and does not generalize well over unseen samples. Meaning that it can only train using pairs of fMRI recordings and their matching clips. Since one of the main challenges is the very limited training data, the generalization abilities of this method are very restricted. 

% % pre-trained action recognition network + self-supervised video representation
% For the task of video reconstruction, we wanted to benefit from pre-trained temporal features in addition to the spatial features. For this purpose, we examined works that focus on video comprehensions, such as video classification or action recognition. In those works, one needs to process the temporal information, in addition to processing the spatial information. Several works have tried to tackle these tasks using two-stream networks - one stream for RGB, and another one for optical flow (OF) \cite{Carreira2017, Stroud2020}. However, these methods require computing the OF in advance, which means that they are not end-to-end networks. Recent works have tried to tackle these tasks using implicit learning of the motion. In a recent work \cite{Crasto2019}, they learned two networks - a teacher network that learns action recognition using OF as an input, and a student network, that receives only RGB input. The student network learns to classify actions based on the RGB input, and the teacher network outputs. At inference time the network uses only the RGB input, meaning that the network learns implicitly the motion input. In another line of work, a better implicit video representation was learned in a self-supervised manner (without manual labels), using a different task that focuses on the temporal dimension. For example, pace prediction \cite{Wang2020,  Benaim2020, Yao2020}, distinguish between ordered and shuffled videos \cite{Misra2016, Fernando2017, Jenni2020} and prediction of the next frame \cite{DPC}. Those works succeed in achieving state-of-the-art results on action recognition and video classification tasks, by employing the implicit video representation they learned. 

%   \begin{figure}[H]%
%         \centering
%         \subfloat{{\includegraphics[width=\textwidth]{Slide15.JPG} }}%

%         \\
%         \subfloat{{\includegraphics[width=\textwidth]{Slide16.JPG} }}%
    
%         \caption{\textbf{Decoder - 1 Hz reconstruction examples - } comparison between the original and reconstructed frames. The 2-4th rows shows reconstructions from subjects 1-3 correspondingly
%         \label{decoder 1Hz fig}}
        
        
%     \end{figure}

% In the following work, we reconstruct the dynamic stimuli, by using novel methods for self-supervision. For this purpose, we use two different networks - an encoder that receives a short video clip and outputs an fMRI sample, and a decoder network that receives one or more fMRI samples and outputs one or more reconstructed video frames. By concatenating these two networks together, encoder-decoder, we obtain a single network, that receives a short video clip and outputs one or more frames. With the concatenated network, we can train the decoder network using clips that do not have matching fMRI. In particular, we can use clips out of the training clips, that are not aligned to any fMRI sample. Moreover, by exploiting the temporal dimension of the data, we enforce temporal continuity over consecutive samples. This by enforcing reconstruction consistency over overlapping (in time) reconstructed frames. 
% The main contributions of this work are: (1) constructing Video Encoder using action recognition features, which succeed better than Encoders based on image classification features. (2) training video decoder using self-supervision which improves the results of supervised approaches and competing methods. (3) Reconstructions temporally consistent video with a higher frame rate relative to the fMRI sampling rate. 
